Locale Encoding For Scalable Multilingual Keyword Spotting Models

A Multilingual Keyword Spotting (KWS) system detects spokenkeywords over multiple locales. Conventional monolingual KWSapproaches do not scale well to multilingual scenarios because ofhigh development/maintenance costs and lack of resource sharing.To overcome this limit, we propose two locale-conditioned universalmodels with locale feature concatenation and feature-wise linearmodulation (FiLM). We compare these models with two baselinemethods: locale-specific monolingual KWS, and a single universalmodel trained over all data. Experiments over 10 localized languagedatasets show that locale-conditioned models substantially improveaccuracy over baseline methods across all locales in different noiseconditions.FiLMperformed the best, improving on average FRRby 61% (relative) compared to monolingual KWS models of similarsizes.

==> Locale Encoding for Universal Model v2/diag.tex <==

\begin{figure}
  \centering
	\begin{tikzpicture}
		\node at (1.5,4){\begin{tabular}{c}input image\\or input feature map\end{tabular}};
	
		\draw (0,0) -- (3,0) -- (3,3) -- (0,3) -- (0,0);
		
		\draw (2,2) -- (2.5,2) -- (2.5,2.5) -- (2,2.5) -- (2,2);
		\draw (2,0.5) -- (2.5,0.5) -- (2.5,1) -- (2,1) -- (2,0.5);
		\draw (1,1) -- (1.5,1) -- (1.5,1.5) -- (1,1.5) -- (1,1);
		
		\draw (2.5,2) -- (7,3.25);
		\draw (2.5,2.5) -- (7,3.25);
 
		\draw (2.5,1) -- (5.75,0.25);
		\draw (2.5,0.5) -- (5.75,0.25);
		
		\draw (1.5,1.5) -- (5.5,1.25);
		\draw (1.5,1) -- (5.5,1.25);
		
		\node at (5.75,4){\begin{tabular}{c}output feature maps\end{tabular}};
		
		\draw[fill=black,opacity=0.2,draw=black] (5.5,1.5) -- (7.5,1.5) -- (7.5,3.5) -- (5.5,3.5) -- (5.5,1.5);
		\draw[fill=black,opacity=0.2,draw=black] (5,1) -- (7,1) -- (7,3) -- (5,3) -- (5,1);
		\draw[fill=black,opacity=0.2,draw=black] (4.5,0.5) -- (6.5,0.5) -- (6.5,2.5) -- (4.5,2.5) -- (4.5,0.5);
		\draw[fill=black,opacity=0.2,draw=black] (4,0) -- (6,0) -- (6,2) -- (4,2) -- (4,0);
	\end{tikzpicture}
	\caption[Illustration of a convolutional layer.]{Illustration of a single convolutional layer. If layer $l$ is a convolutional layer, the input image (if $l = 1$) or a feature map of the previous layer is convolved by different filters to yield the output feature maps of layer $l$.}
	\label{fig:convolutional-layer}
\end{figure}

==> Locale Encoding for Universal Model v2/network.tex <==
\usepackage{xcolor}
\usepackage{xspace}

\definecolor{fc}{HTML}{1E90FF}
\definecolor{h}{HTML}{228B22}
\definecolor{bias}{HTML}{87CEFA}
\definecolor{noise}{HTML}{8B008B}
\definecolor{conv}{HTML}{FFA500}
\definecolor{pool}{HTML}{B22222}
\definecolor{up}{HTML}{B22222}
\definecolor{view}{HTML}{FFFFFF}
\definecolor{bn}{HTML}{FFD700}
\tikzset{fc/.style={black,draw=black,fill=fc,rectangle,minimum height=1cm}}
\tikzset{h/.style={black,draw=black,fill=h,rectangle,minimum height=1cm}}
\tikzset{bias/.style={black,draw=black,fill=bias,rectangle,minimum height=1cm}}
\tikzset{noise/.style={black,draw=black,fill=noise,rectangle,minimum height=1cm}}
\tikzset{conv/.style={black,draw=black,fill=conv,rectangle,minimum height=1cm}}
\tikzset{pool/.style={black,draw=black,fill=pool,rectangle,minimum height=1cm}}
\tikzset{up/.style={black,draw=black,fill=up,rectangle,minimum height=1cm}}
\tikzset{view/.style={black,draw=black,fill=view,rectangle,minimum height=1cm}}
\tikzset{bn/.style={black,draw=black,fill=bn,rectangle,minimum height=1cm}}

\newcommand*{\eg}{\emph{e.g.}\@\xspace}
\newcommand*{\Eg}{\emph{E.g.}\@\xspace}
\newcommand*{\ie}{\emph{i.e.}\@\xspace}
\newcommand*{\etc}{\emph{etc.}\@\xspace}
\newcommand*{\etal}{\emph{et al.}\@\xspace}
\newcommand*{\cf}{\emph{cf.}\@\xspace}
\newcommand*{\vs}{\emph{vs.}\@\xspace}
 
    \node[conv,rotate=90,minimum width=4.5cm] (conv1) at (1.25,0) {\small$\text{conv}_{1, 16, 3}$\,+\,$\text{bn}$\,+\,$\ReLU$};

==> diag.tex <==

\begin{figure}
  \centering
	\begin{tikzpicture}
		\node at (1.5,4){\begin{tabular}{c}input image\\or input feature map\end{tabular}};
	
		\draw (0,0) -- (3,0) -- (3,3) -- (0,3) -- (0,0);
		
		\draw (2,2) -- (2.5,2) -- (2.5,2.5) -- (2,2.5) -- (2,2);
		\draw (2,0.5) -- (2.5,0.5) -- (2.5,1) -- (2,1) -- (2,0.5);
		\draw (1,1) -- (1.5,1) -- (1.5,1.5) -- (1,1.5) -- (1,1);
		
		\draw (2.5,2) -- (7,3.25);
		\draw (2.5,2.5) -- (7,3.25);
 
		\draw (2.5,1) -- (5.75,0.25);
		\draw (2.5,0.5) -- (5.75,0.25);
		
		\draw (1.5,1.5) -- (5.5,1.25);
		\draw (1.5,1) -- (5.5,1.25);
		
		\node at (5.75,4){\begin{tabular}{c}output feature maps\end{tabular}};
		
		\draw[fill=black,opacity=0.2,draw=black] (5.5,1.5) -- (7.5,1.5) -- (7.5,3.5) -- (5.5,3.5) -- (5.5,1.5);
		\draw[fill=black,opacity=0.2,draw=black] (5,1) -- (7,1) -- (7,3) -- (5,3) -- (5,1);
		\draw[fill=black,opacity=0.2,draw=black] (4.5,0.5) -- (6.5,0.5) -- (6.5,2.5) -- (4.5,2.5) -- (4.5,0.5);
		\draw[fill=black,opacity=0.2,draw=black] (4,0) -- (6,0) -- (6,2) -- (4,2) -- (4,0);
	\end{tikzpicture}
	\caption[Illustration of a convolutional layer.]{Illustration of a single convolutional layer. If layer $l$ is a convolutional layer, the input image (if $l = 1$) or a feature map of the previous layer is convolved by different filters to yield the output feature maps of layer $l$.}
	\label{fig:convolutional-layer}
\end{figure}

==> network.tex <==
\usepackage{xcolor}
\usepackage{xspace}

\definecolor{fc}{HTML}{1E90FF}
\definecolor{h}{HTML}{228B22}
\definecolor{bias}{HTML}{87CEFA}
\definecolor{noise}{HTML}{8B008B}
\definecolor{conv}{HTML}{FFA500}
\definecolor{pool}{HTML}{B22222}
\definecolor{up}{HTML}{B22222}
\definecolor{view}{HTML}{FFFFFF}
\definecolor{bn}{HTML}{FFD700}
\tikzset{fc/.style={black,draw=black,fill=fc,rectangle,minimum height=1cm}}
\tikzset{h/.style={black,draw=black,fill=h,rectangle,minimum height=1cm}}
\tikzset{bias/.style={black,draw=black,fill=bias,rectangle,minimum height=1cm}}
\tikzset{noise/.style={black,draw=black,fill=noise,rectangle,minimum height=1cm}}
\tikzset{conv/.style={black,draw=black,fill=conv,rectangle,minimum height=1cm}}
\tikzset{pool/.style={black,draw=black,fill=pool,rectangle,minimum height=1cm}}
\tikzset{up/.style={black,draw=black,fill=up,rectangle,minimum height=1cm}}
\tikzset{view/.style={black,draw=black,fill=view,rectangle,minimum height=1cm}}
\tikzset{bn/.style={black,draw=black,fill=bn,rectangle,minimum height=1cm}}

\newcommand*{\eg}{\emph{e.g.}\@\xspace}
\newcommand*{\Eg}{\emph{E.g.}\@\xspace}
\newcommand*{\ie}{\emph{i.e.}\@\xspace}
\newcommand*{\etc}{\emph{etc.}\@\xspace}
\newcommand*{\etal}{\emph{et al.}\@\xspace}
\newcommand*{\cf}{\emph{cf.}\@\xspace}
\newcommand*{\vs}{\emph{vs.}\@\xspace}
 
    \node[conv,rotate=90,minimum width=4.5cm] (conv1) at (1.25,0) {\small$\text{conv}_{1, 16, 3}$\,+\,$\text{bn}$\,+\,$\ReLU$};
